CANDID: Correspondence AligNment for Deep-burst Image Denoising

With the advent of mobile phone photography and point-and-shoot cameras, deep-burst imaging is widely used for a number of photographic effects such as depth of field, super-resolution, motion deblurring, and image denoising. In this work, we propose to solve the problem of deep-burst image denoising by including an optical flow-based correspondence estimation module which aligns all the input burst images with respect to a reference frame. In order to deal with varying noise levels the individual burst images are pre-filtered with different settings. Exploiting the established correspondences one network block predicts a pixel-wise spatially-varying filter kernel to smooth each image in the original and prefiltered bursts before fusing all images to generate the final denoised output. The resulting pipeline achieves state-of-the-art results by combining all available information provided by the burst.

==> Dockerfile <==
FROM reitzig/texlive-base:2021.10
RUN apk update && apk add --no-cache bash perl python3 py3-pip
RUN pip3 install pygments

# Emulate "Install dependencies" of "entrypoint work ..."
RUN tlmgr update --self --repository http://ftp.math.utah.edu/pub/tex/historic/systems/texlive/2021/tlnet-final
COPY Texlivefile /work/src
RUN xargs tlmgr install --repository http://ftp.math.utah.edu/pub/tex/historic/systems/texlive/2021/tlnet-final < "/work/src/Texlivefile" && \
    sha256sum "/work/src/Texlivefile" > "/work/tmp/Texlivefile.sha" && \
#
# make latexmk and texlogsieve available
    cp /usr/local/texlive/2021/bin/x86_64-linuxmusl/latexmk /usr/local/bin && \
    cp /usr/local/texlive/2021/bin/x86_64-linuxmusl/texlogsieve /usr/local/bin && \
# use latest texlogsieve
    cd /usr/local/bin && wget https://gitlab.com/lago/texlogsieve/-/raw/main/texlogsieve?inline=false


==> _latexmkrc <==
# `-file-line-error` is similar to `--interaction nonstopmode`, but shows the concrete line number
# Remove it, it you want lualatex to stop on errors
$pdflatex = 'pdflatex --shell-escape --interaction nonstopmode --synctex=-1 %O %S | texlogsieve';

#Use SumatraPDF instead of the default PDF viewer
$pdf_previewer = 'start "C:\Program Files\SumatraPDF\SumatraPDF.exe"';

#SumatraPDF updates automatically
$preview_mode = 0;

#automatically call lualatex/pdflatex (instead of latex)
$pdf_mode = 1;

add_cus_dep('glo', 'gls', 0, 'run_makeglossaries');
add_cus_dep('acn', 'acr', 0, 'run_makeglossaries');

sub run_makeglossaries {
  if ( $silent ) {
    system "makeglossaries", "-q", $_[0];
  }
  else {
    system "makeglossaries", $_[0];
  };
}

# enable deletion of *.bbl when calling "latexmk -c"
$bibtex_use = 2;

#remove more files than in the default configuration
@generated_exts = qw(acn acr alg aux code ist fls glg glo gls glsdefs idx ind lof lot out thm toc tpt wrt upa upb synctex);
$clean_ext .= ' %R.ist %R.xdy';

